Coordinated Capacity Reductions and Public Communication in the Airline Industry

We investigate the allegation that legacy U.S. airlines communicated via earnings calls to coordinate with other legacy airlines in offering fewer seats on competitive routes. To this end, we first use text analytics to build a novel dataset on communication among airlines about their capacity choices. Estimates from our preferred specification show that the number of offered seats is 2% lower when all legacy airlines in a market discuss the concept of "capacity discipline." We verify that this reduction materializes only when legacy airlines communicate concurrently, and that it cannot be explained by other possibilities, including that airlines are simply announcing to investors their unilateral plans to reduce capacity, and then following through on those announcements.

==> tables/output/sum-stats_market-sizes_city.tex <==
& \multicolumn{3}{c}{Seats} & \multicolumn{2}{c}{Cap. Discipline} & \multicolumn{2}{c}{Talk Eligible} & \multicolumn{2}{c}{Monopoly Market} & \multicolumn{2}{c}{Missing Report}&\\
\cmidrule(l{.75em}){2-4} \cmidrule(l{.75em}){5-6}\cmidrule(l{.75em}){7-8}\cmidrule(l{.75em}){9-10}\cmidrule(l{.75em}){11-12}
&Mean&SD&Median&Mean&SD&Mean&SD&Mean&SD&Mean&SD&N \\
\midrule
\textbf{Market Participants}&&&&&&&&&&&& \\
Mixed Market&14,919.775&16,107.449&9,381.000&0.115&0.319&0.415&0.493&0.166&0.372&0.224&0.417&478,473 \\
Legacy Market&8,475.512&9,413.635&5,428.000&0.070&0.256&0.254&0.435&0.746&0.435&0.265&0.442&309,155 \\
\midrule
\textbf{Market Size}&&&&&&&&&&&& \\
Small&4,813.287&4,728.536&3,627.000&0.005&0.072&0.028&0.165&0.843&0.363&0.191&0.393&86,878 \\
Medium&8,809.122&8,242.300&6,202.000&0.050&0.218&0.169&0.374&0.542&0.498&0.199&0.400&343,173 \\
Large&17,668.181&17,912.377&11,915.000&0.165&0.371&0.607&0.488&0.141&0.348&0.291&0.454&357,577 \\
\midrule
\textbf{Total}&12,390.312&14,223.136&7,809.000&0.097&0.296&0.352&0.478&0.393&0.488&0.240&0.427&787,628 \\


==> tables/output/tab_airport_mkt-cap-flights.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{Mkt. Capacity}&\multicolumn{1}{c}{Flights}\\
\midrule
Capacity Discipline &     -0.0172&     -0.0221\\
                    &    (0.0089)&    (0.0053)\\
Talk Eligible       &     -0.0243&      0.0652\\
                    &    (0.0215)&    (0.0108)\\
Monopoly Market     &     -0.4518&     -0.3820\\
                    &    (0.0139)&    (0.0081)\\
Market Missing Report&      0.0342&      0.0322\\
                    &    (0.0126)&    (0.0080)\\
\midrule
R-squared           &       0.172&           .\\
Prob $>$ chi2       &           .&       0.000\\
N                   &     614,311&     614,256\\
\bottomrule
\end{tabular}
}


==> tables/output/tab_airport_split-missing.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}\\
                    &\multicolumn{1}{c}{Log Seats}\\
\midrule
Capacity Discipline &     -0.0198\\
                    &    (0.0060)\\
Talk Eligible       &     -0.0404\\
                    &    (0.0144)\\
Monopoly Market     &      0.0168\\
                    &    (0.0114)\\
Missing (Bankrupt)  &      0.0228\\
                    &    (0.0159)\\
Missing (Other)     &      0.0302\\
                    &    (0.0120)\\
\midrule
R-squared           &       0.088\\
N                   &     841,991\\
\bottomrule
\end{tabular}
}


==> tables/output/tab_airport_start-stop.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}\\
                    &\multicolumn{1}{c}{Log Seats}\\
\midrule
Start Talk          &     -0.0424\\
                    &    (0.0064)\\
Continue Talk       &     -0.0217\\
                    &    (0.0072)\\
Stop Talk 1         &     -0.0452\\
                    &    (0.0057)\\
Stop Talk 2         &      0.0033\\
                    &    (0.0053)\\
\midrule
R-squared           &       0.089\\
N                   &     821,876\\
\bottomrule
\end{tabular}
}


==> tmp/manual_results_noMRM_biz_travel_20181216.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}\\
                    &\multicolumn{1}{c}{Log Seats}&\multicolumn{1}{c}{Log Seats}\\
\midrule
Low Business $\times$ Capacity Discipline		& -0.02778	& -0.03243	\\
                    							& (0.01167) & (0.01003)	\\
Medium Business $\times$ Capacity Discipline		& -0.02187	& -0.02659	\\
                    							& (0.00884)	& (0.00691)	\\
High Business $\times$ Capacity Discipline		&  0.01510 	&  0.00598	\\
							                    & (0.01516) & (0.01345)	\\
Talk Eligible       							& -0.12764	& -0.11967	\\
                    							& (0.01593) & (0.01570)	\\
Market Missing Report							&  0.01203	&			\\
							                    & (0.00691) &			\\
Monopoly Market     							&  0.05299	&  0.05219	\\
							                    & (0.01037) & (0.01038)	\\\midrule
R-squared           							& 0.863		& 0.863		\\
N												& 619,848	& 619,848	\\
\bottomrule
\end{tabular}
}


==> tmp/manual_results_noMRM_table4_20181216.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
                    &\multicolumn{1}{c}{(1)}&\multicolumn{1}{c}{(2)}&\multicolumn{1}{c}{(3)}&\multicolumn{1}{c}{(4)}\\
                    &\multicolumn{1}{c}{Log Seats}&\multicolumn{1}{c}{Log Seats}&\multicolumn{1}{c}{Log Seats}&\multicolumn{1}{c}{Log Seats}\\
\midrule

Capacity Discipline 	&  0.00769	& -0.00449		& -0.01240		& -0.02529	\\
                    	& (0.00463) & (0.00415)		& (0.00529)   	& (0.00497)	\\
Talk Eligible       	& -0.11367	& -0.10774		& -0.11522		& -0.10760	\\
                    	& (0.01390) & (0.01367)		& (0.01664)   	& (0.01637)	\\
Market Missing Report	&  0.01943	&				&  0.02673		&			\\
                    	& (0.00517) &				& (0.00563)   	&			\\
Monopoly Market     	&  0.04446	&  0.04323		&  0.04240		&  0.04061	\\
                    	& (0.01013) & (0.01011)		& (0.01075)		& (0.01070)	\\\midrule
R-squared           	&  0.870  	&  0.870			&  0.875			&  0.875	\\
N                   	&  785,939	&  785,938		&  656,288     	&  626,288	\\
\bottomrule
\end{tabular}
}

==> tmp/manual_results_robustness_20190108.tex <==
\begin{tabular}{lllllll}\toprule
								& (1) 			& (2)		& (3)		& (4) 		& (5)		\\
								&  Log Seats		& Log Seats	& Log Seats 	& Log Seats	& Log Seats	\\\midrule
Only $j$ Talks					&  0.03230		&			&			&			&			\\
								& (0.00623)		&			&			&			&			\\
Monopoly Capacity Discipline 	&				&  0.02674	&  0.00835	&			&			\\
								&				& (0.00683)	& (0.00391)	&			&			\\
Capacity Discipline $N-1$		&				&			&			&  0.00249	&			\\
								&				&			&			& (0.00392)	&			\\
Capacity-Discipline-not-$j$		&				&			&			&			&  0.00537	\\
								&				&			&			&			& (0.00641)	\\
Talk Eligible					& -0.12947		& -0.13415	&			& -0.13802	& -0.13790	\\
								& (0.01399)		& (0.01413)	&			& (0.01412)	& (0.01406)	\\
Missing Market Report			& -0.01538		& -0.02148	& -0.01162	& -0.02102	&  0.02196	\\
								& (0.00571)		& (0.00567)	& (0.00613)	& (0.00588)	& (0.0056)	\\
Monopoly Market					&  0.05290		&  0.04602	&			&  0.05422	&  0.05434	\\
								& (0.00924)		& (0.00935)	&			& (0.00923)	& (0.00915)	\\\midrule
R-squared						&  0.866			&  0.866		&  0.869	&  0.866	&  0.866	\\
N								&  840,149		&  840,149	&  439,858	&  840,149	&  840,149	\\\bottomrule
\end{tabular}

